Safe and Interpretable Estimation of Optimal Treatment Regimes

Recent statistical and reinforcement learning methods have significantly advanced patient care strategies. However, these approaches face substantial challenges in high-stakes contexts, including missing data, inherent stochasticity, and the critical requirements for interpretability and patient safety. Our work operationalizes a safe and interpretable framework to identify optimal treatment regimes. This approach involves matching patients with similar medical and pharmacological characteristics, allowing us to construct an optimal policy via interpolation. We perform a comprehensive simulation study to demonstrate the framework's ability to identify optimal policies even in complex settings. Ultimately, we operationalize our approach to study regimes for treating seizures in critically ill patients. Our findings strongly support personalized treatment strategies based on a patient's medical history and pharmacological features. Notably, we identify that reducing medication doses for patients with mild and brief seizure episodes while adopting aggressive treatment for patients in intensive care unit experiencing intense seizures leads to more favorable outcomes.

==> discuss.tex <==
\section{Discussion and Limitations}
\paragraph{Clinical Relevance.} 
\textcolor{red}{SAHAR, BRANDON -- can you help us write this?}

% \paragraph{Methodological Limitations.} Our study, like any causal research, relies on untestable assumptions. We assume there are no hidden variables affecting both EA burden and patient discharge outcomes, though unmeasured disease characteristics might violate this assumption. Additionally, the misspecification of our predefined policy template, intended for doctor interpretability, could affect real-world drug administration, akin to issues discussed in recent work \cite{savje2023causal}. Furthermore, while we focus on point estimation for personalized optimal treatment regimes, handling uncertainty, especially when estimating the exposure map from observed data, remains an open question.

% Like any causal study, our work also depends on untestable assumptions. Here, we assume that there are no hidden variables that simultaneously affect the EA burden and a patient's discharge outcome. This assumption may be violated if there are underlying (unmeasured) disease characteristics that are making a patient predisposed to EA and also affecting brain health. Another potential threat to the validity of our study is the misspecification of the policy template. While our framework is flexible enough and can handle nonparametric policy representation, we use a predefined policy template to ensure interpretability to the doctors. While this template is derived from the hospital protocols, it is likely that in practice the drug administration deviates away from this template. This problem is analogous to the problem of a misspecified exposure map explored in a recent work  \cite{savje2023causal}. Lastly, our work primarily focuses on point estimation of personalized optimal treatment regimes. However, uncertainty quantification in our setup is still an open question, especially when the exposure map (administered regime) is also estimated from the observed data. 

==> introduction.tex <==
\section{Introduction}
Our study focuses on estimating optimal treatment strategies for critically ill patients with seizures or epileptiform activity (EA). EA is observed in over half of patients that undergoing electroencephalography \citep{gaspard2013similarity}, especially critically ill individuals grappling with brain injuries \citep{lucke2015traumatic}, cancer \citep{lee2013risk}, organ failure \citep{boggs2002seizures}, and infections such as COVID-19 \citep{nikbakht2020does}. High levels of EA significantly increase in-hospital mortality, with survivors often experiencing functional or cognitive disabilities \citep{parikh2023effects,ganesan2019electrographic,kim2018}. 

Healthcare professionals currently employ a range of anti-seizure medications (ASMs) to manage EA in intensive care units (ICUs) \citep{farrokh2018antiepileptic}. However, there is concern around the use of highly effective ASMs, such as propofol, due to their adverse long-term effects on patients' health \citep{de2016effect}. For instance, the tragic case of Michael Jackson, the pop artist, highlights the potential dangers of propofol overdose \citep{kim2014trial}. Therefore, it is imperative to carefully design personalized treatment regimens for these patients, with a primary focus on their long-term well-being.

In this retrospective study, we meticulously analyze a cohort of critically ill patients who experienced EA. The dataset was collected at a prominent tertiary hospital from 2016 to 2018. Our primary objective is to identify optimal treatment regimens and assess their potential impact on patient outcomes. Additionally, the process of estimating an optimal treatment regimen serves as an exploratory analysis with the aim of generating hypotheses that can steer future clinical investigations within the domain of critical care \citep{zhang2018interpretable}.

Like many medical studies using retrospective data, our investigation is not without its data challenges. While our dataset includes a substantial cohort of 995 patients, which is considered large within the medical context, it is quite small for many machine-learning methodologies. Furthermore, our data only contains observations within a limited time window for each patient, leaving a substantial portion of each patient's clinical timeline unobserved. Additionally, the intricate interactions between the brain and the administered drugs remain largely unknown, rendering the construction of a reliable pharmacological emulator a formidable challenge due to the inherent stochasticity embedded in our data.

The literature on dynamic treatment regimes and reinforcement learning has been instrumental in addressing scenarios characterized by intricate risk-reward trade-offs among potential treatment choices. These methodologies have found application in optimizing dynamic treatment regimes within healthcare contexts, including but not limited to treatment therapies for HIV and Warfarin treatment post-surgical valve replacement \citep{moodie2007demystifying, chakraborty2014dynamic, zeng2022optimizing}. While reinforcement learning methods such as $\mathcal{Q}$-learning and policy gradient approaches have gained prominence in these areas, their applicability to observational studies akin to ours, replete with the aforementioned data challenges, remains limited \citep{tsiatis2019dynamic, chakraborty2014dynamic, zhang2019reinforcement, zhang2020designing}. Most existing methods in this domain assume experimental data, predefined finite horizons, access to an underlying simulator, countably many state and action spaces, or the absence of missing state-action data. Moreover, many contemporary reinforcement learning techniques are data-hungry and use black-box machine learning methods, rendering them unsuitable for our context. Concerns regarding interpretability and the potential for recommending unsafe actions due to extrapolation further underscore the need for tailored solutions. In Section~\ref{sec: literature} and Appendix~\ref{sec: lit_survey_appendix}, we undertake a comprehensive survey of the existing literature, providing a detailed examination of relevant works in this field.

\paragraph{Contributions.} In this paper, we present a general and flexible framework that allows for consistent estimation of a safe and interpretable optimal treatment regime even under the above-mentioned challenges. Our approach extends the \textit{matching} framework, commonly used for estimating the causal effects, to estimate optimal treatment regime(s). To create a tighter estimation of individualized regimes, our method leverages mechanistic knowledge (such as pharmacological dynamics) to model state-action interaction and distance metric learning to create tight-matched groups. Importantly, our approach confines its estimates to the local neighborhood of observed data, thereby minimizing the risk of unsafe or unreasonable actions. Our framework actively enables domain experts to validate the estimation process through case-based reasoning, enhancing its credibility and applicability. The simplicity and transparency of our approach, coupled with its flexibility and interpretability, make it particularly suited for high-stakes scenarios such as the design of treatment strategies for patients experiencing epileptiform activity (EA) in the ICU. We discuss the identification of optimal treatment regimes in Section~\ref{sec: id} and delineate our methodology to estimate them in Section~\ref{sec: method}.

While none of the existing dynamic treatment regime frameworks or reinforcement learning methodologies are inherently suited for our setup, we have adapted them to align with the specific challenges of our work and compare them with our approach. In Section~\ref{sec: synth}, we provide evidence of the strength of our approach through a straightforward simulation study, inspired by real-world data. This study highlights the significant performance gains our method offers in estimating optimal treatment regimes. 

Using our framework, we analyze our observational study data of ICU patients from a large tertiary hospital in the USA (discussed in Section~\ref{sec: seizure_study}). Optimal treatment regimes recommended by our study highlight clinically important patterns with respect to patients' prognoses and medical history. Specifically, our findings advocate for an aggressive approach to managing high EA burden in critically ill patients with worse prognoses while suggesting reduced drug dosages for patients with mild EA burden for a short duration. These not only help us characterize approaches that help with treating critically ill patients but also generate clinically relevant hypotheses for future inquiry.



==> policy_assignment_alg.tex <==
\begin{algorithm} 
% \label{alg: policy-assignment}
\caption{Algorithm to assign a policy $\pi_i$ to each patient $i$ under policy assignment strategy 5(b).}
\label{alg: policy-assignment}
{\DontPrintSemicolon 
\KwData{Pre-treatment covariates $\mathbf{X}_i$ for each patient $i$.}
\KwResult{Policy $\pi_i$ for each patient $i$.}
\Begin{ 
    \textrm{(Loop over each patient.)}\;
    \For{$i$ in $\{1,\dots,n\}$ }{ 
        \textrm{(Assign random value between 0 and 1)}\;
        $\eta_i\sim\text{Uniform}(0,1)$\;
        
        \textrm{(If neither $\sum_{j=1}^2 X_{i,j}$ nor $\sum_{j=3}^4 X_{i,j}$ are large, assign a moderate policy with high probability.)}\;
        \eIf{$\sum_{j=1}^2 X_{i,j} < 0$ and $\sum_{j=3}^4 X_{i,j} < 0$}
        { 
            \eIf{ $\eta_i < 0.1$ }
            {
                $\pi_i \leftarrow \pi^a_i$\;
            }{
            \eIf{ $\eta_i < 0.9$ }{
                $\pi_i \leftarrow \pi^m_i$\;
            }{ 
            $\pi_i \leftarrow \pi^c_i$\;
            }
            }
        }{
            \textrm{(Else If $\sum_{j=1}^2 X_{i,j}$ > $\sum_{j=3}^4 X_{i,j}$, assign an aggressive policy with high probability.)}\;
            \eIf{$\sum_{j=1}^2 X_{i,j} > \sum_{j=3}^4 X_{i,j}$}
            { 
            \eIf{ $\eta_i < 0.8$ }
            {
                $\pi_i \leftarrow \pi^a_i$\;
            }{
            \eIf{ $\eta_i < 0.9$ }{
                $\pi_i \leftarrow \pi^m_i$\;
            }{ 
            $\pi_i \leftarrow \pi^c_i$\;
            }
            }
            }
            {\textrm{(Else If $\sum_{j=1}^2 X_{i,j} \leq \sum_{j=3}^4 X_{i,j}$, assign a conservative policy with high probability.)}
            
            \eIf{ $\eta_i < 0.1$ }
            {
                $\pi_i \leftarrow \pi^a_i$\;
            }{
            \eIf{ $\eta_i < 0.2$ }{
                $\pi_i \leftarrow \pi^m_i$\;
            }{ 
            $\pi_i \leftarrow \pi^c_i$\;
            }
            }                    
            }
        
        }
        
        
    }
}
}
% \caption{Algorithm to assign a policy $\pi_i$ to each patient $i$ under policy assignment strategy 5(b).}
% \label{alg: policy-assignment}
\end{algorithm}

==> synth_data_res.tex <==
\begin{table}
\centering
\begin{tabular}{l l l l l l l l l l l l l} 
Covs & T& T Drop& Binary& DGP & Observed & Our Method & Expert & Linear Q-learning& DTree Q-learning& Linear Q-learning& RF Q-learning& SV Q-learning\\
10 & 1 & 1 & \ding{55} & semi-random & 0.40 & 0.22 & 0.36 & 0.69 & 0.69 & 0.72 & 0.60 & 0.54 \\
10 & 1 & 2 & \ding{55} & semi-random & 0.40 & 0.21 & 0.36 & 0.54 & 0.54 & 0.55 & 0.56 & 0.52 \\
10 & 2 & 1 & \ding{55} & semi-random & 0.28 & 0.21 & 0.24 & 0.67 & 0.67 & 0.71 & 0.60 & 0.72 \\
10 & 2 & 2 & \ding{55} & semi-random & 0.28 & 0.20 & 0.24 & 0.75 & 0.75 & 0.75 & 0.59 & 0.57 \\
10 & 1 & 1 & \ding{51} & semi-random & 0.36 & 0.36 & 0.34 & 0.43 & 0.43 &  &  &  \\
10 & 1 & 2 & \ding{51} & semi-random & 0.36 & 0.50 & 0.34 & 0.45 & 0.45 &  &  &  \\
10 & 2 & 1 & \ding{51} & semi-random & 0.39 & 0.35 & 0.35 & 0.63 & 0.63 &  &  &  \\
10 & 2 & 2 & \ding{51} & semi-random & 0.39 & 0.35 & 0.35 & 0.61 & 0.61 &  &  &  \\
100 & 1 & 1 & \ding{55} & semi-random & 0.39 & 0.20 & 0.35 &  &  & 0.68 & 0.61 & 0.54 \\
100 & 1 & 2 & \ding{55} & semi-random & 0.39 & 0.20 & 0.35 & 0.56 & 0.56 & 0.60 & 0.62 & 0.53 \\
100 & 2 & 1 & \ding{55} & semi-random & 0.27 & 0.21 & 0.24 &  &  & 0.67 & 0.60 & 0.73 \\
100 & 2 & 2 & \ding{55} & semi-random & 0.28 & 0.20 & 0.24 &  &  & 0.72 & 0.64 & 0.68 \\
\end{tabular}
\end{table}
